Deformed Mirror Symmetry for Punctured Surfaces

Mirror symmetry originally envisions a correspondence between deformations of the A-side and deformations of the B-side. In this paper, we achieve an explicit correspondence in the case of punctured surfaces. The starting point is the noncommutative mirror equivalence $ \operatorname{Gtl} Q \cong \operatorname{mf} (\operatorname{Jac} \check{Q}, \ell) $ for a punctured surface $ Q $. We pick a deformation $ \operatorname{Gtl}_q Q $ which captures a large part of the deformation theory and includes the relative Fukaya category. To find the corresponding deformation of $ \operatorname{mf} (\operatorname{Jac} \check{Q}, \ell) $, we deform work of Cho-Hong-Lau which interprets mirror symmetry as Koszul duality. As result we explicitly obtain the corresponding deformation $ \operatorname{mf} (\operatorname{Jac}_q \check{Q}, \ell_q) $ together with a deformed mirror functor $ \operatorname{Gtl}_q Q \xrightarrow{\sim} \operatorname{mf} (\operatorname{Jac}_q \check{Q}, \ell_q) $. The bottleneck is to verify that the algebra $ \operatorname{Jac}_q \check{Q} $ is indeed a (flat) deformation of $ \operatorname{Jac} \check{Q} $. We achieve this by deploying a result of Berger-Ginzburg-Taillefer on deformations of CY3 algebras, which however requires the relations to be homogeneous. We show how to replace this homogeneity requirement by a simple boundedness condition and obtain flatness of $ \operatorname{Jac}_q \check{Q} $ for almost all $ Q $. We finish the paper with examples, including a full treatment of the 3-punctured sphere and 4-punctured torus. With the help of our computations in arXiv:2305.09112, we describe $ \operatorname{Jac}_q \check{Q} $ explicitly. It turns out that the deformed potential $ \ell_q $ is still central in $ \operatorname{Jac}_q \check{Q} $, in contrast to the popular slogan that central elements do not survive under deformation.

==> MS/fig_Abousign.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
\newcommand{\basicgrid}{%
\path[draw] (0, 0) -- ++(right:1) coordinate[midway] (1-0) -- ++(right:1) coordinate[midway] (3-0) -- ++(right:1) coordinate[midway] (5-0);
\path[draw] (0, 1) -- ++(right:1) coordinate[midway] (1-2) -- ++(right:1) coordinate[midway] (3-2) -- ++(right:1) coordinate[midway] (5-2);
\path[draw] (0, 2) -- ++(right:1) coordinate[midway] (1-4) -- ++(right:1) coordinate[midway] (3-4) -- ++(right:1) coordinate[midway] (5-4);
\path[draw] (0, 3) -- ++(right:1) coordinate[midway] (1-6) -- ++(right:1) coordinate[midway] (3-6) -- ++(right:1) coordinate[midway] (5-6);
\path[draw] (0, 0) -- ++(up:1) coordinate[midway] (0-1) -- ++(up:1) coordinate[midway] (0-3) -- ++(up:1) coordinate[midway] (0-5);
\path[draw] (1, 0) -- ++(up:1) coordinate[midway] (2-1) -- ++(up:1) coordinate[midway] (2-3) -- ++(up:1) coordinate[midway] (2-5);
\path[draw] (2, 0) -- ++(up:1) coordinate[midway] (4-1) -- ++(up:1) coordinate[midway] (4-3) -- ++(up:1) coordinate[midway] (4-5);
\path[draw] (3, 0) -- ++(up:1) coordinate[midway] (6-1) -- ++(up:1) coordinate[midway] (6-3) -- ++(up:1) coordinate[midway] (6-5);
}
%
\newcommand{\zigzaglags}{%
\path[draw, thick] plot[smooth] coordinates{($ (0-1)!-0.5!(1-2) $) (0-1) ($ (0-1)!0.5!(1-2) + (315:0.1) $) (1-2) ($ (1-2)!0.5!(2-3) + (135:0.1) $) (2-3) ($ (2-3)!0.5!(3-4) + (315:0.1) $) (3-4) ($ (3-4)!0.5!(4-5) + (135:0.1) $) (4-5) ($ (4-5)!0.5!(5-6) + (315:0.1) $) (5-6) ($ (5-6)!-0.5!(4-5) $)};
\path[draw, thick] plot[smooth] coordinates{($ (0-3)!-0.5!(1-4) $) (0-3) ($ (0-3)!0.5!(1-4) + (315:0.1) $) (1-4) ($ (1-4)!0.5!(2-5) + (135:0.1) $) (2-5) ($ (2-5)!0.5!(3-6) + (315:0.1) $) (3-6) ($ (3-6)!-0.5!(2-5) $)};
\path[draw, thick] plot[smooth] coordinates{($ (0-5)!-0.5!(1-6) $) (0-5) ($ (0-5)!0.5!(1-6) + (315:0.1) $) (1-6) ($ (1-6)!-0.5!(0-5) $)};
\path[draw, thick] plot[smooth] coordinates{($ (1-0)!-0.5!(2-1) $) (1-0) ($ (1-0)!0.5!(2-1) + (135:0.1) $) (2-1) ($ (2-1)!0.5!(3-2) + (315:0.1) $) (3-2) ($ (3-2)!0.5!(4-3) + (135:0.1) $) (4-3) ($ (4-3)!0.5!(5-4) + (315:0.1) $) (5-4) ($ (5-4)!0.5!(6-5) + (135:0.1) $) (6-5) ($ (6-5)!-0.5!(5-4) $)};
\path[draw, thick] plot[smooth] coordinates{($ (3-0)!-0.5!(4-1) $) (3-0) ($ (3-0)!0.5!(4-1) + (135:0.1) $) (4-1) ($ (4-1)!0.5!(5-2) + (315:0.1) $) (5-2) ($ (5-2)!0.5!(6-3) + (135:0.1) $) (6-3) ($ (6-3)!-0.5!(5-2) $)};
\path[draw, thick] plot[smooth] coordinates{($ (5-0)!-0.5!(6-1) $) (5-0) ($ (5-0)!0.5!(6-1) + (135:0.1) $) (6-1) ($ (6-1)!-0.5!(5-0) $)};
\path[draw, thick] plot[smooth] coordinates{($ (0-1)!-0.5!(1-0) $) (0-1) ($ (0-1)!0.5!(1-0) + (45:0.1) $) (1-0) ($ (1-0)!-0.5!(0-1) $)};
\path[draw, thick] plot[smooth] coordinates{($ (0-3)!-0.5!(1-2) $) (0-3) ($ (0-3)!0.5!(1-2) + (45:0.1) $) (1-2) ($ (1-2)!0.5!(2-1) + (225:0.1) $) (2-1) ($ (2-1)!0.5!(3-0) + (45:0.1) $) (3-0) ($ (3-0)!-0.5!(2-1) $)};
\path[draw, thick] plot[smooth] coordinates{($ (0-5)!-0.5!(1-4) $) (0-5) ($ (0-5)!0.5!(1-4) + (45:0.1) $) (1-4) ($ (1-4)!0.5!(2-3) + (225:0.1) $) (2-3) ($ (2-3)!0.5!(3-2) + (45:0.1) $) (3-2) ($ (3-2)!0.5!(4-1) + (225:0.1) $) (4-1) ($ (4-1)!0.5!(5-0) + (45:0.1) $) (5-0) ($ (5-0)!-0.5!(4-1) $)};
\path[draw, thick] plot[smooth] coordinates{($ (1-6)!-0.5!(2-5) $) (1-6) ($ (1-6)!0.5!(2-5) + (225:0.1) $) (2-5) ($ (2-5)!0.5!(3-4) + (45:0.1) $) (3-4) ($ (3-4)!0.5!(4-3) + (225:0.1) $) (4-3) ($ (4-3)!0.5!(5-2) + (45:0.1) $) (5-2) ($ (5-2)!0.5!(6-1) + (225:0.1) $) (6-1) ($ (6-1)!-0.5!(5-2) $)};
\path[draw, thick] plot[smooth] coordinates{($ (3-6)!-0.5!(4-5) $) (3-6) ($ (3-6)!0.5!(4-5) + (225:0.1) $) (4-5) ($ (4-5)!0.5!(5-4) + (45:0.1) $) (5-4) ($ (5-4)!0.5!(6-3) + (225:0.1) $) (6-3) ($ (6-3)!-0.5!(5-4) $)};
\path[draw, thick] plot[smooth] coordinates{($ (5-6)!-0.5!(6-5) $) (5-6) ($ (5-6)!0.5!(6-5) + (225:0.1) $) (6-5) ($ (6-5)!-0.5!(5-6) $)};
}
%
\basicgrid
\path[fill, color=gray!50] plot[smooth] coordinates{(3-0) ($ (3-0)!0.5!(4-1) + (135:0.1) $) (4-1) ($ (4-1)!0.5!(5-2) + (315:0.1) $) (5-2) ($ (5-2)!0.5!(6-3) + (135:0.1) $) (6-3)} -- plot[smooth] coordinates{(6-3) ($ (5-4)!0.5!(6-3) + (225:0.1) $) (5-4) ($ (4-5)!0.5!(5-4) + (45:0.1) $) (4-5) ($ (3-6)!0.5!(4-5) + (225:0.1) $) (3-6)} -- plot[smooth] coordinates{(3-6) ($ (2-5)!0.5!(3-6) + (315:0.1) $) (2-5) ($ (1-4)!0.5!(2-5) + (135:0.1) $) (1-4) ($ (0-3)!0.5!(1-4) + (315:0.1) $) (0-3)} -- plot[smooth] coordinates{(0-3) ($ (0-3)!0.5!(1-2) + (45:0.1) $) (1-2) ($ (1-2)!0.5!(2-1) + (225:0.1) $) (2-1) ($ (2-1)!0.5!(3-0) + (45:0.1) $) (3-0)};
\basicgrid
\zigzaglags
\end{tikzpicture}
\caption{A midpoint polygon with four sides of length three}
\label{fig:MS-defsuperpotential-Abousign}


==> examples/fig_torus_large.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.8\linewidth}
\centering
\begin{tikzpicture}[scale=2]
\newcommand{\arrowbetween}[2]{($ (#1)!0.1!(#2) $) -- ($ (#2)!0.1!(#1) $)}
\newcommand{\thetorus}{%
% horizontal
\path[draw, ->] \arrowbetween{0, 0}{1, 0} node[midway, above] {$ a_1 $};
\path[draw, ->] \arrowbetween{2, 0}{1, 0} node[midway, above] {$ a_2 $};
\path[draw, ->] \arrowbetween{0, 2}{1, 2} node[midway, above] {$ a_1 $};
\path[draw, ->] \arrowbetween{2, 2}{1, 2} node[midway, above] {$ a_2 $};
\path[draw, ->] \arrowbetween{1, 1}{0, 1} node[midway, above] {$ a_3 $};
\path[draw, ->] \arrowbetween{1, 1}{2, 1} node[midway, above] {$ a_4 $};
%
\path[draw, ->] \arrowbetween{0, 1}{0, 0} node[midway, left] {$ b_1 $};
\path[draw, ->] \arrowbetween{0, 1}{0, 2} node[midway, left] {$ b_3 $};
\path[draw, ->] \arrowbetween{2, 1}{2, 0} node[midway, left] {$ b_1 $};
\path[draw, ->] \arrowbetween{2, 1}{2, 2} node[midway, left] {$ b_3 $};
\path[draw, ->] \arrowbetween{1, 0}{1, 1} node[midway, left] {$ b_2 $};
\path[draw, ->] \arrowbetween{1, 2}{1, 1} node[midway, left] {$ b_4 $};
%
\path (0, 0) node {\small $ 1 $};
\path (2, 0) node {\small $ 1 $};
\path (2, 2) node {\small $ 1 $};
\path (0, 2) node {\small $ 1 $};
\path (1, 0) node {\small $ 2 $};
\path (1, 2) node {\small $ 2 $};
\path (0, 1) node {\small $ 3 $};
\path (2, 1) node {\small $ 3 $};
\path (1, 1) node {\small $ 4 $};}
%
\begin{scope}[shift={(2, 0)}, every path/.style={gray}] \thetorus \end{scope}
\begin{scope}[shift={(2, 2)}, every path/.style={gray}] \thetorus \end{scope}
\begin{scope}[shift={(2, 4)}, every path/.style={gray}] \thetorus \end{scope}
\begin{scope}[shift={(4, 0)}, every path/.style={gray}] \thetorus \end{scope}
\begin{scope}[shift={(4, 2)}, every path/.style={gray}] \thetorus \end{scope}
\begin{scope}[shift={(4, 4)}, every path/.style={gray}] \thetorus \end{scope}
\begin{scope}[shift={(0, 0)}, every path/.style={gray}] \thetorus \end{scope}
\begin{scope}[shift={(0, 2)}, every path/.style={gray}] \thetorus \end{scope}
\begin{scope}[shift={(0, 4)}, every path/.style={gray}] \thetorus \end{scope}
\end{tikzpicture}
\caption{Large torus}
\end{subfigure}
\end{figure}


==> prelim-koszul/backup_prop.tex <==
\begin{proof}
An element of $ \Hom_{\rModfd} (ℂ, ℂ) $ is simply a coderivation $ ℂ ¤ T(\bar A[1]) → ℂ ¤ T(\bar A[1]) $ and an element of $ \koszul A $ is a linear map $ T(\bar A[1]) → ℂ $. Projecting a coderivation down to its zeroth component gives a correspondence between the two. On vector spaces level, this is our desired isomorphism:
\begin{align*}
Ψ: \Hom_{\rModfd} (ℂ, ℂ) &\isoto \koszul A \\
f &↦ f_0.
\end{align*}
As usual, we have used here $ T(\bar A[1]) $ for coderivations instead of $ T(A[1]) $. Both domain and codomain of $ Ψ $ are dg algebras and we intend to show that $ Ψ $ preserves their differential and product.

Let us check that $ Ψ $ preserves the differential. Pick a coderivation $ f: ℂ ¤ T(\bar A[1]) → ℂ ¤ T(\bar A[1]) $. Recalling that $ μ_ℂ = 0 $, the differential $ μ^1_{\rModfd A} (f) $ reduces to commuting with $ μ_A $ and we get
\begin{align*}
Ψ(μ^1_{\rModfd A} (f)) = (μ_A ∘ f - (-1)^{|f|} f ∘ μ_A)_0 = - (-1)^{|f|} f ∘ μ_A = d_{\koszul A} f.
\end{align*}
This shows that $ Ψ $ preserves differentials and explains the somewhat mysterious sign of $ d_{\koszul A} $ chosen in \autoref{def:koszul-koszul-def}.

Next, let $ g: ℂ ¤ T(\bar A[1]) → ℂ ¤ T(\bar A[1]) $ be another coderivation. It is our aim to show $ (f ∘ g)_0 = f_0 g_0 $ as elements of $ \koszul A $. Assume for simplicity that $ f $ is supported only on tensors of length $ s $ and that $ g $ is supported only tensors of length $ t $. Let us put
\begin{align*}
Φ: \kdual{(\bar A[1]^{¤ s})} ¤ \kdual{(\bar A[1]^{¤ t})} &\verylongisoto \kdual{(\bar A[1]^{¤ t} ¤ \bar A[1]^{¤ s})}, \\
a ¤ b &\verylongmapsto (-1)^{|a||b|} (w ¤ v ↦ b(w) a(v)).
\end{align*}
By \autoref{def:koszul-koszul-def}, we have $ f_0 g_0 = Φ(f_0 ¤ g_0) $. For every $ w ∈ \bar A[1]^{¤ s} $ and $ v ∈ \bar A[1]^{¤ t} $ we get
\begin{align*}
(f ∘ g)_0 (w ¤ v) &= f_0 ((-1)^{|g||v|} g_0 (w) · v) = (-1)^{|g||v|} g_0 (w) f_0 (v) \\
&= Φ(f_0 ¤ g_0)(w ¤ v) = (f_0 g_0) (w ¤ v).
\end{align*}
Note we have used that $ |f| = |v| $. We conclude
\begin{equation*}
Ψ(μ^2_{\rModfd A} (f, g)) = (f ∘ g)_0 = f_0 g_0 = Ψ(f) Ψ(g).
\end{equation*}
This shows that $ Ψ $ provides a dg isomorphism between $ \koszul A $ and $ \Hom_{\rModfd} (ℂ, ℂ) $, finishing the proof.
\end{proof}


==> prelim-koszul/remarks.tex <==
Goal:
• A! CY dg algebra
• explain arising of CHL-type functor in case End(L) is really pos. graded cyclic
Mod End(L) → Tw \H^0\koszul A.
• Explain \H^0\koszul A is CY3 if this functor is qi.
• Or show \H^0 \koszul A is CY if \koszul A is dg CY.
This is not the case, but merely a guess.
Indeed, A! always CY under cyclicity assu on A. But H^0 A! not always CY.

\begin{definition}
Let $ A $ be a dg algebra. A \emph{$ A $-bimodule} is a graded vector space $ M $ together with a left-$ A $ action and a right $ A $-action which commute.
\end{definition}

The dg algebra $ A^{\env} $ is defined as
\begin{align*}
d(x ¤ y) &= dx ¤ y + (-1)^{‖x‖} x ¤ dy,
%%μ^2 (x ¤ y, x' ¤ y') &= (-1)^{|y||x'| + |x'| + |y'|} xx' ¤ yy'
μ^2 (x ¤ y, x' ¤ y') &= (-1)^{|y||x'|} μ^2 (x, x') ¤ μ^2 (y, y').
\end{align*}
We claim that $ A^{\env} $ is a dg algebra this way. Indeed,
\begin{equation*}
d(d(x ¤ y)) = d(dx ¤ y + (-1)^{‖x‖} x ¤ dy) \\
= d(d(x)) ¤ y + (-1)^{|x|} dx ¤ dy + (-1)^{‖x‖} dx ¤ dy + (-1)^{‖x‖ + ‖x‖} x ¤ d(d(y)) = 0.
d(μ^2 (x ¤ y, x' ¤ y')) = (-1)^{|y||x'|} d(μ^2 (x, x') ¤ μ^2 (y, y'))
= (-1)^{|y||x'|} (d μ^2 (x, x') ¤ μ^2 (y, y') + (-1)^{|xx'|} μ^2 (x, x') ¤ d μ^2 (y, y')) \\
= (-1)^{|y||x'|} [((-1)^{1 + ‖x'‖} μ^2 (dx, x') ¤ μ^2 (y, y') + (-1)^{1} μ^2 (x, dx') ¤ μ^2 (y, y'))
+ (-1)^{|xx'|} (μ^2 (x, x') ¤ (-1)^{1} μ^2 (y, dy') + μ^2 (x, x') ¤ (-1)^{1 + ‖y'‖} μ^2 (dy, y'))] \\
while
(-1)^{|x'| + |y'|} μ^2 (d(x ¤ y), x' ¤ y') + μ^2 (x ¤ y, d(x' ¤ y')) \\
= (-1)^{|x'| + |y'|} ((-1)^{|y||x'|} μ^2 (dx, x') ¤ μ^2 (y, y') + (-1)^{|x| + |dy||x'|} μ^2 (x, x') ¤ μ^2(dy, y'))
+ ((-1)^{|y||dx'|} μ^2 (x, dx') ¤ μ^2 (y, y') + (-1)^{|x'| + |y||x'| μ^2 (x, x') ¤ μ^2 (y, dy')).
\end{equation*}
This is equivalent to 

\begin{definition}
Let $ A $ be an $ A_∞ $-algebra and $ M $ a graded vector space together with degree $ 1-(i+j) $ maps
\begin{equation*}
μ: A^{¤i} ¤ M ¤ A^{¤j} → M.
\end{equation*}
Requirement is … (direct signs?)
\end{definition}

\begin{definition}
Let $ A $ be an $ A_∞ $-algebra. Then $ A[1] ¤ A[1] $ becomes an $ A $-bimodule by [direct construction].
\end{definition}
We have quoted the signs from \cite[Remark 1.7]{Mescher}.

\begin{remark}
Let $ A $ be a dg algebra (with the signs of $ A_∞ $-algebras). Then we put $ A^{\env} = A[1] ¤ A[1] $. It is an $ A $-bimodule ("outer action").
\end{remark}

\begin{definition}
Let $ A $ be an $ A_∞ $-algebra and $ M $ an $ A_∞ $-bimodule over $ A $. Then $ M[d] $ is the bimodule over $ A $ given by [sign flip].
μ(a_k, …, sm, …, a_1) = (-1)^{‖a_1‖ + … + ‖a_s‖} μ(a_k, …, m, …, a_1)?
\end{remark}

\begin{remark}
The inner action also exists in the $ A_∞ $-context.
\end{remark}

\begin{definition}
Let $ A $ be an $ A_∞ $-algebra. Let $ M $ be an $ A_∞ $-bimodule over $ A $. Then $ \Hom_{A^{\env}} (M, A^{\env}) $ is naturally an $ A $-bimodule with the action given by the inner action on $ A^{\env} $.
\end{definition}

\begin{definition}
A morphism of $ A $-bimodules is a map such that […]. It is a quasi-isomorphism if $ F^1 $ is a quasi-isomorphism of complexes.
\end{definition}

%-----

\begin{definition}
An $ A_∞ $-bimodule $ M $ is $ μ_M: T(A) ¤ M ¤ T(A) → T(A) ¤ M ¤ T(A) $ two-sided coderivation (biderivation?) such that $ μ_M + μ_A $ squares to zero. Here $ μ_A $ denotes left and right application of $ μ_A $ product.
%%%%An $ A_∞ $-bimodule $ M $ is module $ μ_{M, l}: T(A)_{>0} ¤ M → T(A) ¤ M $ and $ μ_{M, r}: M ¤ T(A)_{>0} → M ¤ T(A) $ and $ μ_{M, m}: M → M $ such that $ μ_{A, l} + μ_{A, r} + μ_{M, l} + μ_{M, r} + μ_{M, m} $ squares to zero.
\end{definition}

\begin{definition}
Let $ A $ be an $ A_∞ $-category. The category $ \Bimod A $ of $ A $-bimodules is the dg category defined as follows:
\begin{itemize}
\item Objects are the $ A $-bimodules $ (M, μ_M) $.
\item Hom spaces are biderivations $ f: T(A) ¤ M ¤ T(A) → T(A) ¤ N ¤ T(A) $.
\item Composition is standard.
\item Differential of $ f $ is
\begin{equation*}
μ^1 (f) = (μ_A + μ_N) ∘ f - f ∘ (μ_A + μ_M).
\end{equation*}
\end{itemize}
\end{definition}

\begin{lemma}
$ \Bimod A $ is a dg category.
\end{lemma}

\begin{proof}
Standard. We have $ μ^1 (μ^1 (f)) = (μ_A + μ_N) ∘ f ∘ (μ_A + μ_M) - (μ_A + μ_N) ∘ f ∘ (μ_A + μ_M) + (μ_A + μ_N) ∘ (μ_A + μ_N) ∘ f + f ∘ (μ_A + μ_M) ∘ (μ_A + μ_M) = 0 $.
\end{proof}

\begin{remark}
A morphism of bimodules is a closed degree zero morphism in the dg category $ \Bimod A $. As always, a dg category comes with a notion of quasi-isomorphisms.
\end{remark}

Not all $ A_∞ $-algebras have a finite free bimodule resolution. Can we say projective here?

\begin{definition}
Let $ A $ be an $ A_∞ $-algebra with a finite free bimodule resolution $ P^• ∈ \Tw\Bimod A $. Then the hom space
\begin{equation*}
\Hom_{\Bimod A} (P^k, A^{\env})
\end{equation*}
enjoys a bimodule structure by regarding the inner structure on $ A^{\env} $. We denote this complex of modules by $ \Ext_{A^{\env}}^• (A, A^{\env}) $. It is an element of $ \Tw\Bimod A $.
\end{definition}

Note: Let C a dg category. Then Ch^b (C) ⊂ Tw C. Yeah, here we take Ch^b (C) as $ A_∞ $-category.
Note: This "Ext" is denoted RHom in the literature.

\begin{definition}
Let $ A $ be a dg algebra. Then $ A $ is \CYn\ if there is a quasi-isomorphism of elements of $ \Tw\Bimod A $
\begin{equation*}
\Ext_{A^{\env}} (A, A^{\env}) ≅ A[n].
\end{equation*}
\end{definition}

\begin{remark}
Let $ A $ be a \CYn\ dg algebra. Then $ \HH^k (A, A^{\env}) = δ_{kn} A $. Indeed, this Hochschild cohomology is computed by the complex $ \Hom_{\Bimod A} (P^•, A^{\env}) $. By assumption this complex has cohomology $ A $ concentrated in degree $ n $. Proves the claim.
\end{remark}

\begin{lemma}
If $ A $ is a degree $ n $ $ A_∞ $-Frobenius algebra, then the dg algebra $ \koszul A $ is \CYn.
\end{lemma}

\begin{proof}
As $ A_∞ $-algebras we have $ A ≅ A^* [n] $ hence $ \koszul A 
\end{proof}


%--- BTW
In fact, we claim that if $ A $ is cylic of degree $ n = 3 $, then the relations $ dx $ are precisely derivatives of a superpotential. So let us assume $ n = 3 $ and denote by $ ⟨-, -⟩ $ the pairing of $ A $. Pick a graded basis $ \id, x_1, …, x_n, x_1^*, …, x_n^*, \coid $ for $ A $, where $ x_i $ are elements in degree $ 1 $ and $ x_i^* $ their dual elements of degree $ 2 $ corresponding via $ ⟨-, -⟩ $. Define the superpotential $ W $ according to [construction]:
\begin{equation*}
W ∈ ℂ⟨x_1, …, x_n, x_1^*, …, x_n^*⟩.
Now define $ W' $ as the superpotential obtained by restricting $ W $ to paths only containing of basis elements $ x_i $ of degree $ 1 $. We claim that the ideal $ I $ is precisely generated by the derivatives $ ∂_{x_i} W' $. In fact, we claim that $ d \kdual{(x_i^*)} = ∂_{x_i} W $. Indeed, the let $ 1 ≤ i_1, …, i_k ≤ n $ be indices. Then for the $ x_{i_k} … x_{i_k} $-coefficient of $ ∂_{x_i} W $ and $ d \kdual{(x_i^*)} $ we observe
\begin{equation*}
∂_{x_i} W' \restr_{x_{i_k} … x_{i_1}} = ⟨μ(x_{i_k}, …, x_{i_1}), x_i⟩ = (d \kdual{(x_i^*)}) \restr_{x_{i_k} … x_{i_1}}.
\end{equation*}
This shows $ d \kdual x_i = ∂_{x_i^*} W' $ and the ideal $ I $ is precisely $ I(\{∂_{x_i^*} W'\})_{\compl{T(\kdual{(A^1)})}} $. In conclusion, if $ n = 3 $ then the generators of the desired ideal $ I $ are precisely the derivatives of $ W $.

The unique feature of the case $ n = 3 $ is that the scalars in the superpotential are $ ⟨μ(x_{i_k}, …, x_{i_1}), x_i⟩ $ which are nonvanishing for $ x_{i_1}, …, x_{i_k} $, $ x_i $ of degree $ 1 $. If $ n $ were not $ 3 $, then we cannot naturally represent the ideal $ I $ by means of a superpotential $ W' ∈ \compl{T(\kdual{(A^1)})} $. Indeed, the derivative $ ∂_x W' $ contains only variables in $ \koszul A $ that are of degree $ 0 $. Correspondingly, for an element $ x ∈ \kdual A $ we can express $ dx $ in terms of $ W' $ if and only if $ x $ is of degree 1.

